TextMI: Textualize Multimodal Information for Integrating Non-verbal Cues in Pre-trained Language Models

Pre-trained large language models have recently achieved ground-breaking performance in a wide variety of language understanding tasks. However, the same model can not be applied to multimodal behavior understanding tasks (e.g., video sentiment/humor detection) unless non-verbal features (e.g., acoustic and visual) can be integrated with language. Jointly modeling multiple modalities significantly increases the model complexity, and makes the training process data-hungry. While an enormous amount of text data is available via the web, collecting large-scale multimodal behavioral video datasets is extremely expensive, both in terms of time and money. In this paper, we investigate whether large language models alone can successfully incorporate non-verbal information when they are presented in textual form. We present a way to convert the acoustic and visual information into corresponding textual descriptions and concatenate them with the spoken text. We feed this augmented input to a pre-trained BERT model and fine-tune it on three downstream multimodal tasks: sentiment, humor, and sarcasm detection. Our approach, TextMI, significantly reduces model complexity, adds interpretability to the model's decision, and can be applied for a diverse set of tasks while achieving superior (multimodal sarcasm detection) or near SOTA (multimodal sentiment analysis and multimodal humor detection) performance. We propose TextMI as a general, competitive baseline for multimodal behavioral analysis tasks, particularly in a low-resource setting.

==> draft.tex <==
Multimodal models for understanding human communication need a proper representation of text, audio, and facial expressions. Many tasks often have small datasets and cannot be well trained with raw audio-visual features. We introduce Multimodal-CLIP that jointly learns to represent acoustic and visual features from a human speech video in a self-supervised manner. Contrastive loss allows aligning video segments with corresponding audio while ensuring unrelated video and audios are well separated. We experiment on several multimodal benchmark datasets to show diverse applications of the pre-trained model. Multimodal-CLIP embeddings help zero-shot similar video retrieval and speaker identification in CMU-MOSI. Combined with a pre-trained language model, Multimodal-CLIP can be fine-tuned for a diverse range of communication tasks that require multimodal understanding. Experiments on humor and sarcasm detection show performance improvement when the acoustic-visual network is initialized with pre-trained weights.
